When More Reformulations Hurt: Avoiding Drift using Ranker Feedback

Modern retrieval pipelines increasingly rely on query reformulation and neural reranking to improve effectiveness, but this comes at a significant computational cost and introduces a fundamental tradeoff between recall and query drift. Generating many reformulated queries can substantially increase recall, yet naively merging or exhaustively reranking their results is prohibitively expensive. In this work, we argue that the core challenge is not reformulation generation itself, but the adaptive selection of reformulations and their retrieved documents under a strict inference budget. We propose ReformIR, a budget-aware retrieval framework that treats query reformulations as first-class features and performs online relevance estimation using a strong reranker as a teacher. Given multiple reformulated queries, ReformIR constructs a large candidate pool and learns a lightweight surrogate model that estimates document utility from reformulation-specific retrieval signals. Under a fixed reranking budget, the surrogate adaptively prioritizes both reformulations and documents, selectively querying a teacher reranker anchored to the original query. This process increases recall while actively suppressing drift through online feature selection over reformulations. We conduct extensive experiments on the MSMARCO passage corpora and TREC Deep Learning benchmarks (DL19-DL22). Our results show that ReformIR consistently outperforms existing reformulation strategies, particularly as the number of reformulations increases, where prior methods suffer from severe quality degradation due to drift. Our findings also suggest a shift in retrieval system design, rather than using large language models as rerankers, their capacity is more effectively leveraged in the reformulation stage with feedback-driven optimization.

==> alg-cascade.tex <==
\begin{algorithm}[t]
\caption{Cascading Two-Level Bandit for RAG with Intermediate Surrogate Updates}
\label{alg:cascading}
\begin{algorithmic}[1]
\REQUIRE Query $x$, reformulations $\mathcal{Q}$, document pool $\mathcal{D}$, threshold $\tau$, confidence $\beta_t$, weight $\eta$
\FOR{$t = 1$ to $T$}
    \STATE Extract reformulation features $\{\phi_q\}$ for $q \in \mathcal{Q}$
    \STATE \textbf{Level-1 selection:}
    \[
    q_t = \arg\max_q \left[\phi_q^\top \hat{\theta}_{t-1} + c_1 \sqrt{\phi_q^\top V_{t-1}^{-1} \phi_q}\right]
    \]
    \STATE Generate candidate subsets $\mathcal{S}_{q_t}$ for $q_t$
    \FOR{each $S \in \mathcal{S}_{q_t}$}
        \STATE Compute $\hat{u}(S) = \psi_S^\top \hat{\omega}_{t-1}$ and 
        $\sigma(S) = \sqrt{\psi_S^\top W_{t-1}^{-1} \psi_S}$
    \ENDFOR
    \STATE Select $S_t = \arg\max_S \hat{u}(S) - \beta_t \sigma(S)$
    \STATE \textbf{Intermediate Level-1 update:} use $\hat{u}(S_t)$ to update Level-1 with weight $\eta$
    \STATE \textbf{Threshold check:}
    \IF{$\hat{u}(S_t) - \beta_t \sigma(S_t) \ge \tau$}
        \STATE Call LLM with $(q_t, S_t)$ to get $y_t$ and $r_t = r_{\mathrm{LLM}}(y_t)$
        \STATE Update Level-2 with $(\psi_{S_t}, r_t)$
        \STATE Update Level-1 with $(\phi_{q_t}, r_t)$ (full weight)
    \ELSE
        \STATE Update Level-2 with surrogate $(\psi_{S_t}, \hat{u}(S_t))$
    \ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> fig/qualitative.tex <==
\definecolor{myPink}{RGB}{210, 168, 182}
\definecolor{myTeal}{RGB}{120, 164, 172}

\definecolor{baselineColor}{RGB}{240, 244, 248} % Soft Slate Blue/Gray
\definecolor{baselineBorder}{RGB}{176, 190, 197}
\definecolor{oursColor}{RGB}{232, 245, 233}    % Soft Emerald
\definecolor{oursBorder}{RGB}{129, 199, 132}
\definecolor{oursText}{RGB}{46, 125, 50}
\definecolor{paperNavy}{RGB}{30, 55, 100}
\definecolor{innerFill}{RGB}{248, 250, 252}  % <--- New: Very pale gray-blue for the dashed box

\begin{figure}[ht]
    \centering
    \resizebox{\columnwidth}{!}{
        \begin{tikzpicture}[
            node distance = 0cm,
            % Define standard box style
            font=\Huge,
            baseBox/.style={
                rectangle, 
                draw=baselineBorder, 
                fill=baselineColor, 
                rounded corners=3pt, 
                line width=0.8pt,
                text width=14cm, 
                inner sep=10pt, 
                anchor=north west,
                align=left
            },
            dashedBox/.style={
                rectangle,
                draw=paperNavy!60, % Slightly faded navy
                dashed,
                dash pattern=on 8pt off 5pt,
                line width=1.5pt,
                rounded corners=6pt,
                fill=white, % White background makes text pop inside the blue box
                text width=13cm,
                inner sep=15pt,
                align=left
            },
            % Style for your method
            oursBox/.style={
                baseBox,
                draw=oursBorder,
                fill=oursColor,
                line width=1.2pt
            }
        ]

        % Top Box (Baselines)
        \node[baseBox] (top) at (0, 0) {
            {\textbf{Initial Query:}} 
            \texttt{supartz injections what does it made of }\\[1.2em]
            \textbf{Reformulations:}  \\[.2em]
            \begin{tikzpicture}
            \node[dashedBox] {
            \textbf{Query 1:} question: What are the ingredients used in Supartz injections? answer:... \\
            \textit{Initial Recall@50:} \textbf{0.32} \\[1em]
            \textbf{Query 2:} How is Supartz formulated and what components does it contain? answer:... \\
            \textit{Initial Recall@50:} \textbf{0.18} \\[1.em]
            \textbf{Query 3:} What is the purpose of each ingredient in Supartz injections? answer:... \\
            \textit{Initial Recall@50:} \textbf{0.16} 
                        };
        \end{tikzpicture} \\[1.em]
        \textbf{QA-Expand (baseline)} \textit{Recall@50} : \textcolor{red}{0.265}
        };

        % Bottom Box (Ours) - Positioned with a small gap
        \node[oursBox, below=0.2cm of top] (bottom) {
            {\textbf{\textcolor{oursText}{QA-Expand + ReformIR (Ours):}}} \\
            \textit{Query 1 learned weight:  \textbf{0.99}, Query 2 learned weight: \textbf{0.1}, Query 3 learned weight: \bf{0.1e-7}}

            \textit{Final Recall@50:} \textbf{0.368}
        };

        \end{tikzpicture}
    }
    \caption{Comparison between standard query reformulations and our proposed \textbf{ReformIR} approach. }
    \label{fig:reformir_improved}
\end{figure}




==> fig2.tex <==
\tikzset{
  stage/.style n args={2}{
    align=left,
    text width=0.86\columnwidth,
    inner sep=0.8em,
    rounded corners=2pt,
    draw=black,
    line width=0.5pt,
    fill=#1,
    label={
      [fill=black, rounded corners=2pt, font=\sffamily\scriptsize,
       text=white, anchor=west, xshift=-6.0em, inner sep=0.25em]above:#2
    },
  },
  desc/.style={
    align=right,
    text width=10.5em,
    font=\small,
  },
  identifier/.style={font=\small},
  stepnum/.style={
    circle,
    fill=black,
    text=white,
    font=\small\bfseries,
    inner sep=0.2em,
    outer sep=0.2em,
  },
  arrow/.style={-{Latex[length=2.2mm,width=1.6mm]}, thick},
  dashedarrow/.style={-{Latex[length=2.2mm,width=1.6mm]}, thick, dashed},
  looplabel/.style={font=\footnotesize, inner sep=1pt, fill=white, rounded corners=1pt},
}

\begin{figure}[t]
\centering
\begin{tikzpicture}[node distance=6mm]

% ---- Color palette (subtle, print-friendly) ----
\definecolor{cQuery}{RGB}{235,245,255}
\definecolor{cRetr}{RGB}{237,248,233}
\definecolor{cSur}{RGB}{255,247,230}
\definecolor{cTeach}{RGB}{255,235,238}
\definecolor{cOut}{RGB}{245,245,245}

% =======================
% Left-side descriptors + step numbers
% =======================
\node[desc] (D0) {\textbf{Input}};
\node[stepnum, right=0.25 of D0] (S0) {};

\node[desc, below=14mm of D0] (D1) {\textbf{Recall expansion}\\via reformulations};
\node[stepnum, right=0.25 of D1] (S1) {1};

\node[desc, below=17mm of D1] (D2) {\textbf{Drift control}\\via online selection};
\node[stepnum, right=0.25 of D2] (S2) {2};

\node[desc, below=17mm of D2] (D3) {\textbf{Output}};
\node[stepnum, right=0.25 of D3] (S3) {3};

% =======================
% Main pipeline blocks
% =======================
\node[stage={cQuery}{Query}] (Q) at ($(S0.east)+(1.4,0)$)
{\textbf{Original query}\hfill{\identifier{$Q$}}};

\node[stage={cQuery}{Reformulate}, below=of Q] (R)
{\textbf{Reformulator $\mathcal{R}$ (cheap, short-context)}\par
Generate $m$ reformulations:\par
$\mathcal{Q}=\{Q_1,\ldots,Q_m\}$.};

\node[stage={cRetr}{Retrieve}, below=of R] (RET)
{\textbf{First-stage retrieval (BM25)}\par
Per reformulation: $D_i=\mathrm{Top}k(Q_i)$ for $i=1,\ldots,m$.\par
Union pool (high recall): $\mathcal{C}=\bigcup_{i=1}^{m} D_i$.};

\node[stage={cSur}{Select \& score}, below=of RET] (SUR)
{\textbf{Surrogate model (reformulations as features)}\par
$\Phi(d)=\big[\mathrm{BM25}(Q_1,d),\ldots,\mathrm{BM25}(Q_m,d),\mathrm{BM25}(Q,d)\big]$.\par
Score: $s(d;\mathbf{w})=\mathbf{w}^{\top}\Phi(d)$ (online feature selection).};

\node[stage={cTeach}{Teacher feedback}, below=8mm of SUR] (T)
{\textbf{Teacher reranker $\mathcal{T}$ (budget $B$)}\par
Select $(Q_i,d)$ with bandit/ORE, then query teacher:\par
$y=\mathcal{T}(Q,d)$ for selected $d\in\mathcal{C}$.\par
Update $\mathbf{w}$ online using $(\Phi(d),y)$.};

\node[stage={cOut}{Rank}, below=of T] (OUT)
{\textbf{Final ranking}\par
Return documents by sorting $d\in\mathcal{C}$ using $s(d;\mathbf{w})$.};

% =======================
% Arrows (main flow + loop)
% =======================
\draw[arrow] (Q) -- (R);
\draw[arrow] (R) -- (RET);
\draw[arrow] (RET) -- (SUR);
\draw[arrow] (T) -- (OUT);

% Feedback loop: select and update (right and left routes to avoid overlaps)
\draw[arrow] (SUR.east) -- ++(0.8,0) |- node[looplabel, pos=0.22]
{select $(Q_i,d)$} (T.east);
\draw[dashedarrow] (T.west) -- ++(-0.8,0) |- node[looplabel, pos=0.22]
{update $\mathbf{w}$} (SUR.west);

\end{tikzpicture}
\vspace{-2mm}
\caption{One-column overview of \approach{}. Multiple reformulations increase recall via per-reformulation pools $D_i$ and their union $\mathcal{C}=\bigcup_i D_i$. Drift is suppressed by treating reformulations as features and using budgeted teacher feedback $y=\mathcal{T}(Q,d)$ anchored to the original query to learn weights $\mathbf{w}$ via online feature selection and budget-aware sampling.}
\label{fig:approach_pipeline}
\vspace{-2mm}
\end{figure}

==> intro-OLD.tex <==
\section{Introduction}

Large language models (LLMs) have rapidly become a dominant component in modern
retrieval pipelines, primarily through their use as powerful rerankers.
Applied in a pointwise or listwise fashion, LLM-based rerankers can significantly
outperform traditional neural rankers such as MonoT5, achieving state-of-the-art
effectiveness on benchmarks including BEIR and TREC.
However, these gains come at a steep cost.
Reranking requires the LLM to read and reason over full document texts, and inference
cost scales linearly with the number of candidates.
As a result, even moderately deep reranking (e.g., 50--100 documents) incurs high
latency and monetary expense, placing exhaustive LLM-based reranking beyond the reach
of many practical systems.

This raises a fundamental question for retrieval system design:
\emph{where should expensive language models be used in the pipeline?}
We argue that using LLMs as end-stage judges is often the wrong answer.
Instead, LLMs are far more cost-effective when used upstream for
\emph{query reformulation}.

Generating multiple reformulations requires only short prompts and short outputs, consumes orders of magnitude fewer tokens than document reranking, and leverages the strong query understanding already encoded in modern LLMs.
Crucially, query reformulation does not require large context windows or deep document-level reasoning, making it feasible even with relatively small or lightly fine-tuned language models.

Recent work on LLM-based query expansion and reformulation supports this intuition:
reformulated queries can substantially improve first-stage recall and downstream
task performance at minimal cost.
However, simply generating more reformulations is not sufficient.
While multiple reformulations increase recall, they also introduce a major failure
mode: \emph{query drift}~\cite{rocchio1971relevance}.
Some reformulations capture genuinely relevant aspects of the user’s intent,
while others emphasize tangential or misleading facets, pulling retrieval toward
irrelevant regions of the corpus.
Prior approaches typically merge reformulations statically, via concatenation,
rank fusion, or pseudo-relevance feedback, implicitly assuming that all
reformulations are equally useful.
This assumption is fragile and often leads to degraded precision despite higher recall.

In this work, we argue that the central challenge is not reformulation generation,
but \emph{reformulation selection}.
Each reformulated query should be viewed as a hypothesis about the user’s true intent.
The key question is which hypotheses lead to relevant documents and which induce drift.
We show that this question can be answered efficiently using a small amount of
downstream relevance feedback, without resorting to exhaustive reranking.

We introduce \approach{}, a retrieval framework that uses LLMs exclusively as
\emph{low-cost reformulation generators} and employs a budgeted reranker only as a
teacher to guide selection.
\approach{} generates multiple reformulations, retrieves documents independently
for each reformulation to maximize recall, and then learns, under a strict budget,
which reformulations are useful.
Reformulations are treated as features in a surrogate relevance model, and a
bandit-style optimization loop allocates a limited number of reranker calls to
progressively focus on documents retrieved by promising reformulations.
Importantly, the reranker always evaluates relevance with respect to the original
query, anchoring optimization and actively suppressing query drift.

This design yields several advantages.
First, it decouples query understanding from expensive document-level reasoning.
LLMs are used where they are strongest and cheapest: for understanding and rephrasing
queries, rather than where they are most costly.
Second, because reformulation operates in a short-context regime, \approach{}
naturally supports the use of smaller language models, enabling further reductions
in inference cost.
Third, the framework is generator-agnostic and can be layered like an adapter on top of any
reformulation method; our experiments show consistent improvements across a wide
range of generators.
Finally, by learning explicit weights over reformulations, \approach{} provides
interpretability, revealing which aspects of a query actually drive relevance.

Overall, our work advocates a shift in how LLMs are integrated into retrieval systems.
Rather than treating them as expensive rerankers applied late in the pipeline, we
show that \emph{LLMs are most effective when used early, as low-cost generators of
query hypotheses, combined with lightweight, budget-aware optimization to control
drift}.
This perspective has direct implications for building scalable and cost-efficient
retrieval systems that still benefit from the representational power of modern
language models.

\section{Intro-v2}

==> method.tex <==
\input{fig3}


\section{Method}
\label{sec:method}



In this section we describe our approach in detail...

\subsection{Preliminaries}
\label{sec:preliminaries}

Let $Q$ denote a user query and $\mathcal{D}$ a document collection.
Modern retrieval systems increasingly rely on generating multiple query reformulations
to improve recall, especially for complex or ambiguous queries.
However, while multiple reformulations increase coverage, they also introduce a
well-known failure mode: \emph{query drift}.
Some reformulations retrieve genuinely relevant documents,
while others pull the retrieval process toward tangential or irrelevant regions of the corpus. Our core insight is the following:

\begin{quote}
\emph{High recall requires many reformulations, but high precision requires adaptively identifying and ignoring reformulations that induce drift.}
\end{quote}

The challenge is therefore not reformulation generation itself,
but deciding \emph{which reformulations to prioritize}, and doing so efficiently.
We address this by treating reformulations as features and
using a strong reranker—anchored to the \emph{original query} as a teacher
to dynamically select and weight reformulations under a strict budget.


\subsection{Overview of the \approach{} Pipeline}
\label{sec:overview}

\approach{} is a retrieval pipeline designed to achieve the best of both worlds:
\textbf{high recall from multiple reformulations} and
\textbf{low drift through adaptive, budget-aware selection}.
Figure~\ref{fig:reformopt} provides an overview.

The pipeline consists of four stages:
\begin{enumerate}
    \item generation of multiple query reformulations to increase recall,
    \item retrieval of a large candidate pool across reformulations,
    \item online feature selection over reformulations using a surrogate model,
    \item budgeted interaction with a teacher reranker to arrest drift.
\end{enumerate}

Crucially, the teacher reranker always evaluates relevance with respect to
the \emph{original query} $Q$, providing a stable semantic anchor
that prevents the system from drifting toward reformulation-specific artifacts.


\subsection{Reformulations as Recall-Enhancing Hypotheses}
\label{sec:reformulation}

Given an input query $Q$, a reformulator $\mathcal{R}$ produces a set of
$m$ reformulated queries:
\[
\mathcal{Q} = \{Q_1, Q_2, \ldots, Q_m\}.
\]

Each $Q_i$ captures a distinct hypothesis about the user’s intent,
such as alternative phrasings, subtopics, or domain-specific terminology.
We deliberately generate multiple reformulations—even at the cost of noise—
because this substantially increases recall.

However, not all reformulations are beneficial:
some retrieve relevant documents,
while others induce drift by emphasizing spurious aspects of the query.
Rather than attempting to pre-filter reformulations,
we retain all of them and defer selection to a later, evidence-driven stage.

Importantly, reformulations are never merged or concatenated.
Each $Q_i$ is preserved as an independent signal whose usefulness must be learned.

\subsection{Multi-Reformulation Candidate Pool Construction}
\label{sec:candidate_retrieval}

Each reformulated query $Q_i$ is issued independently to a first-stage retriever
(BM25), producing a ranked list:
\[
D_i = \{d_{i1}, d_{i2}, \ldots, d_{ik}\}.
\]

\input{reformopt_algorithm}
The overall candidate pool is defined as:
\[
\mathcal{C} = \bigcup_{i=1}^{m} D_i \cup R_0.
\]

where $R_0$ is the initial retrieved pool from original query. This union operation is essential for recall:
any document retrievable by any reformulation is retained.
At the same time, it dramatically increases the risk of drift,
since $\mathcal{C}$ may contain documents retrieved by reformulations
that only weakly align with the original query.

We cap $k$ per reformulation to keep $|\mathcal{C}|$ tractable,
but deliberately allow $\mathcal{C}$ to be large enough
to expose the recall–drift tradeoff.

\subsection{Surrogate Model: Reformulations as Features}
\label{sec:surrogate}

To control drift without sacrificing recall, we frame the problem as a top-$l$ arm selection problem in linear stochastic bandits setting \cite{reda2021top}. The arms here correspond to documents in the candidate pool. Linear stochastic bandits model the reward for arms as a linear model of features and estimate utility for each arm suing this linear surrogate approximating the rewards.  
We construct a surrogate relevance model that performs
\emph{online feature selection over reformulations}.

For each document $d \in \mathcal{C}$, we define a feature vector:
\[
\vec x(d) =
\big[
\text{BM25}(Q_1,d), \ldots, \text{BM25}(Q_m,d),
\text{BM25}(Q,d), \text{RM3}(Q`,d)
\big].
\]
While BM25 features capture the relevance of the document to each reformulation, the RM3 features capture the proximity of a document to a small set of documents already deemed relevant by the cross-encoder based ranker $\psi$ (teacher).
%Each feature corresponds directly to a reformulated query.
The surrogate model takes the form:
\[ \textsc{UtilEst}(d; \vec w) = 
s(d; \vec w) = \vec w^\top \vec x(d),
\]
where $\vec{w}$ are the weights that would be estimated and determines the importance assigned to reformulations and helps prioritize documents to rank. Note that the weights assign utility / importance to individual reformulation based features and the overall score estimated for the document determines the utility of the document and determines whether it would be prioritized for ranking using $\psi$ compared to other documents. Hence, ranking of documents occurs adaptively where documents and implicitly reformulations are prioritized leveraging the utility /relevance scores estimated by the surrogate. 

Learning $\mathbf{w}$ is equivalent to learning
\emph{which reformulations increase recall without inducing drift}.
Reformulations that consistently retrieve documents judged relevant
by the teacher receive higher weight,
while drift-inducing reformulations are automatically suppressed.

After sampling the ranker feedback, the estimation error, which measures the discrepancy between the estimated relevance score (\textsc{UtilEst}) and the actual relevance score (\(\psi\)), is calculated. The error is defined as:
\begin{equation}  
\mathcal{E}(\vec{w}; q, d, \vec{x}_d) = \frac{1}{2} \left| \psi(q, d) - \textsc{UtilEst}\left(\vec{w}, \vec{x}_d\right) \right|^2
\end{equation}

 The parameters $\vec w$ are updated to minimize this error.
 
 Note that our setup is inspired by \textbf{disposable bandits} \cite{disposable_bandits}, where a budget on number of times each arm can be sampled, is imposed. In our setup each document can be sampled only once as once it is ranked by $\psi$ Our setup further has an overall budget on the total number of arm samplings which is the re-ranking budget $c$.   
 
\subsection{Budget-Aware Teacher-Guided Optimization}
\label{sec:bandit}

Evaluating all documents in $\mathcal{C}$ with a strong reranker is infeasible.
Instead, we treat the reranker as a \emph{teacher} and interact with it selectively.

We use MonoT5 as the teacher $\mathcal{T}$,
which evaluates relevance with respect to the original query $Q$.
This ensures that all feedback remains grounded in the true information need.

Given a fixed budget $B$ of teacher calls,
we perform a bandit-style optimization over reformulations.
Each reformulation $Q_i$ corresponds to an arm,
and pulling an arm corresponds to selecting a document retrieved by $Q_i$.

At each iteration:
\begin{enumerate}
    \item Select a reformulation $Q_i$ based on current surrogate weights and uncertainty.
    \item Select a document $d \in D_i$ whose relevance is uncertain or promising.
    \item Query the teacher to obtain:
    \[
    y = \mathcal{T}(Q, d).
    \]
    \item Update $\mathbf{w}$ using $(\psi(d), y)$.
\end{enumerate}

This process achieves two goals simultaneously:
\begin{itemize}
    \item \textbf{Drift control}: reformulations that retrieve irrelevant documents are rapidly down-weighted.
    \item \textbf{Efficiency}: limited feedback is concentrated on promising reformulations.
\end{itemize}


\subsection{Why \approach{} Works}
\label{sec:why}

\paragraph{Recall without drift.}
Multiple reformulations dramatically increase recall,
but naïvely using them causes drift.
\approach{} preserves recall while actively suppressing drift
through teacher-guided reformulation selection.

\paragraph{Budget-aware learning.}
Even partial reranking feedback is sufficient:
the surrogate learns from a small number of teacher calls
to prioritize documents from promising reformulations.

\paragraph{Generator-agnostic design.}
Because reformulations are treated as features,
\approach{} can be layered on top of any reformulation generator.
Our experiments show consistent gains across methods
precisely because drift—not generation quality—is the dominant failure mode.

\paragraph{Interpretability.}
The learned weights $\mathbf{w}$ provide direct insight into
which reformulations (and thus which aspects of the query)
were actually responsible for successful retrieval.

%\input{fig}



==> methods_v2_old.tex <==
\input{fig3}

\section{Our Approach \approach{}}
\label{sec:method}


In this section, we present our approach in detail, addressing the challenges of using multiple query reformulations for retrieval. Our aim is to achieve the high recall afforded by many reformulations while maintaining high precision by avoiding query drift. An overview of the pipeline is shown in Figure~\ref{fig:method}.

\subsection{Preliminaries and Problem Setup}

Let $Q$ be the original user query expressing an information need, and let $\mathcal{D}$ be a large document collection. Modern retrieval systems often generate multiple reformulations of $Q$ (alternative phrasings, expansions, etc.) to improve recall, especially for complex or ambiguous queries. The benefit is that different reformulations can retrieve different relevant documents. The drawback is a well-known issue of \textit{query drift}: some reformulations might stray from the user’s intent, retrieving off-target documents~\cite{turtle1995query}. 
Our core insight is that:

\begin{quote}
\emph{High recall requires many reformulations, but high precision requires adaptively identifying and ignoring reformulations that induce drift.}
\end{quote}

In other words, generating a wide range of reformulated queries is only half the battle; the key challenge is deciding which reformulations (and their results) to prioritize and which to down-weight or ignore. We tackle this by treating reformulations as latent features of the retrieval process and using a strong reranker, anchored to the original query, as a guide (or “teacher”) to dynamically select and weight reformulations under a strict budget of reranker evaluations.

\subsection{Overview of the \approach{} Pipeline}

Our proposed pipeline, called \approach{}, is designed to get the best of both worlds: it leverages multiple query reformulations for high recall and employs adaptive selection to minimize drift. The pipeline consists of four main stages:

\subsubsection{Reformulation Generation} Produce a set of $m$ reformulated queries from the original query $Q$. These reformulations ${Q_1, Q_2, \ldots, Q_m}$ aim to cover various interpretations or aspects of the query, increasing the chance of retrieving all relevant information.
    
\subsubsection{Candidate Retrieval} Use a first-stage retriever (we use BM25) to execute each reformulated query $Q_i$ and obtain a list of top-$k$ documents $D_i = {d_{i1}, d_{i2}, \ldots, d_{ik}}$. The initial results for the original query $Q$ (denoted $R_0$) are also obtained. All retrieved documents are combined into a candidate pool:

    $$
\mathcal{C} \;=\; R_0 \;\cup\; \bigcup_{i=1}^{m} D_i~,$$

where $\mathcal{C}$ may contain duplicate documents if the same document appears in multiple $D_i$ (in practice, such duplicates are de-duplicated in the set union). This union operation ensures maximal recall — any document that is highly ranked for any reformulation or for the original query will be considered. However, $\mathcal{C}$ can be quite large and potentially noisy, since some reformulations might pull in irrelevant content. We typically cap the depth $k$ of each list to keep $|\mathcal{C}|$ manageable, while still allowing $\mathcal{C}$ to be large enough to include most relevant documents. Figure~\ref{fig:method} (right side) illustrates this multi-reformulation retrieval process.
    
\subsubsection{Surrogate Model (Reformulations as Features)} We embed reformulations into a feature-based surrogate model that can predict document relevance. Instead of deciding upfront which reformulations are useful, we assign each reformulation a weight that will be learned from data. Concretely, for each document $d \in \mathcal{C}$, we construct a feature vector $\mathbf{x}_d$ with one dimension for each reformulated query’s contribution to $d$. 

\[
  x_d =
\big[
\text{BM25}(Q_1,d), \ldots, \text{BM25}(Q_m,d),
\text{BM25}(Q,d), \text{RM3}(Q`,d)
\big].
\]

% For example, $\mathbf{x}_d$ can include features like:

%     \begin{itemize}
%         \item BM25 score of $d$ for query $Q_1$,
%         \item   BM25 score of $d$ for $Q_2$, …,
%         \item   BM25 score of $d$ for $Q_m$,
%         \item   BM25 score of $d$ for the original query $Q$,
%         \item   An RM3 feedback score of $d$ w.r.t. an expanded query $Q’$.
%     \end{itemize}
    
This way, each reformulation $Q_i$ is represented as a feature indicating how well document $d$ matches that particular query. The original query’s BM25 score is also included as a feature, and we add an RM3-based feature to capture pseudo-relevance feedback signals. In our implementation, $Q’$ for RM3 is an expanded version of the original query $Q$ computed using a small set of documents ($S1$) already identified as relevant by the teacher (initially, this could be the top results from $R_0$, and it can be updated as more feedback comes in). The RM3 feature for document $d$ is essentially the query-likelihood or relevance model score of $d$ under this expanded query $Q’$, which measures the vocabulary overlap between $d$ and the known relevant set. Intuitively, while the BM25 features capture direct term overlap with each query formulation, the RM3 feature captures indirect relevance: it indicates whether $d$ shares terms with other documents that were judged relevant, thereby serving as a drift-resistant signal.

\subsection{Surrogate Relevance Model}

We denote our surrogate relevance model as a linear function 
$s(d; \mathbf{w})$ that estimates the relevance of document $d$ given the feature vector:
$$s(d; \mathbf{w}) \;=\; \mathbf{w}^\top \mathbf{x}_d~$$,
where $\mathbf{w}$ is a weight vector (of dimension $m$ + a few additional features) that the model will learn. Each component of $\mathbf{w}$ corresponds to the importance of the associated feature (and thereby the associated reformulation or original query or feedback signal). Initially, we can start with $\mathbf{w}$ set to some default (e.g., zero or small random values). Learning $\mathbf{w}$ is effectively learning which reformulations (or signals) are useful: if reformulation $Q_i$ tends to retrieve relevant documents, the weight $w_i$ will increase; if $Q_i$ retrieves mostly irrelevant documents, $w_i$ will decrease (potentially becoming negative if that reformulation is consistently misleading).
We frame this \textit{surrogate model learning problem} in terms of an \textit{online learning} or bandit problem. 

\subsection{Modeling documents as multi-arm bandits}

In a multi-armed bandit scenario, each arm is an option that can be tried (here, think of each document or reformulation as an ``arm''), and the goal is to maximize reward by sequentially selecting arms and learning from feedback. 
In our setting: Each candidate document $d \in \mathcal{C}$ can be considered an arm with an unknown true relevance reward (which we can only observe by asking the expensive teacher $\psi$).  The feature vector $\mathbf{x}_d$ is known for each arm $d$ without asking the teacher (it’s computed from query similarities like BM25 scores). 
We assume there is an unknown weight vector $\mathbf{w}$ such that the expected reward of document $d$ (i.e., the teacher’s judgment of relevance) is approximately $\mathbf{w}^{\top}\mathbf{x}_d$. This is the standard linear bandit assumption – it means our linear surrogate model is capable of predicting relevance if we find the right weights.
The challenge is to learn $\mathbf{w}$ by sampling a limited number of arms (documents to send to the teacher) and observing their rewards (teacher scores). This is akin to a stochastic linear bandit problem, where each teacher evaluation provides a noisy signal of the true relevance.

To learn $\mathbf{w}$, we define a loss function that quantifies the error in our surrogate’s predictions. Whenever the teacher $\psi$ evaluates a document $d$ for query $Q$, we get a relevance score or label $y = \psi(Q,d)$ (e.g., a relevance score from MonoT5). We want our surrogate to predict this value. For a given weight vector $\mathbf{w}$, the estimation error for document $d$ can be written as:
\begin{equation}
\label{eq:loss}
\mathcal{E}(\mathbf{w}; Q, d, \mathbf{x}_d) = \frac{1}{2}\Big( \psi(Q,d) -s(d;\mathbf{w}) \Big)^2~
\end{equation}
The surrogate model’s goal is to find weights $\mathbf{w}$ that minimize this error for the documents that have been evaluated by the teacher so far.
This setup draws inspiration from the linear bandit and online regression that has also been used in document ranking recently~\cite{online-bandits,ore} [add citation here]. 
In particular, since each document (arm) can only be evaluated once by the teacher (we don’t revisit the same document twice), our setting can be seen as an instance of ``disposable bandits''\cite{disposable_bandits}, where each arm is ``used up'' after one pull. 
We also impose a strict overall budget $c$ on the total number of teacher calls, so the learning process must be very sample-efficient.

\todo{should we discuss the merits of disposable bandits??}

\todo{add retrieval after reformulation in figure 1}

\subsection{Budget-Aware Teacher-Guided Optimization}

Once we have the candidate pool $\mathcal{C}$ and the surrogate model structure in place, the next step is to select which documents to send to the teacher for evaluation, under the constraint that we can only afford $B$ teacher evaluations. Our strategy is an iterative, feedback-driven selection that uses the surrogate model to decide which documents (and implicitly which reformulations) to focus on. The procedure is summarized in Algorithm~\ref{algo:cerberus}.

At a high level, each iteration of the process does the following:

\begin{enumerate}

    \item 
\textbf{ Surrogate-based Relevance estimation:} Evaluate the current surrogate model $s(d;\mathbf{w}_t)$ on all remaining candidate documents $d \in \mathcal{C}$. This gives each candidate an estimated relevance score. Initially, when $\mathbf{w}_1$ is untrained, these scores may be uninformative (e.g., all zero or random), but as we incorporate feedback, they become more accurate.
    
    \item  \textbf{Select a Batch of Documents:} Identify a batch $B$ of the top $b$ highest-scoring documents according to the surrogate (i.e., the $b$ documents most likely to be relevant). Here $b$ is a batch size parameter that can be as small as 1 (one document at a time) or larger for efficiency. We ensure this selection respects the remaining budget; for example, if fewer than $b$ evaluations are left, we schedule that amny documents. (In our experiments we set a moderate batch size so that we update weights in small increments, balancing learning efficiency and computational parallelism.)

    \item  \textbf{Teacher Evaluation:} Send the selected documents $B$ to the teacher (re-ranker) $\psi$ for relevance evaluation. The teacher (MonoT5 in our case) scores each document in $B$ with respect to the original query $Q$, producing a relevance score or label for each. These teacher scores $y_d = \psi(Q,d)$ are the “ground truth” signals that will guide the surrogate.
    
    \item
     \textbf{Surrogate Update:} Update the surrogate model’s weight vector $\mathbf{w}$ using the new feedback. We adjust $\mathbf{w}$ to minimize the error $\mathcal{E}$ (Equation \ref{eq:loss}) for the documents in $B$. In practice, this could be done by stochastic gradient descent on the loss, a closed-form least squares solution if we aggregate all seen examples, or other online regression techniques. The key point is that weights for features (reformulations) that contributed to correctly retrieving a relevant document will increase, while weights corresponding to reformulations that retrieved non-relevant documents will decrease. This online feature selection aspect means the model is gradually identifying which reformulations are useful.
    
    \item \textbf{Repeat: }Remove the batch $B$ from the candidate pool $\mathcal{C}$ (since those documents have now been handled) and add them to the result list $R_1$ (along with their teacher scores). Then repeat the scoring and selection process for the next iteration, with the updated model $\mathbf{w}_{t+1}$, until we exhaust the budget $B$ or there are no more candidates.

\end{enumerate}

This iterative process continues until we have used up our budget of teacher calls (i.e., we have obtained $\psi$ scores for $B$ documents in total). The end product is a set $R_1$ of up to $B$ documents, each with a relevance score given by the teacher. We can then produce the final ranked list by sorting $R_1$ according to the teacher’s scores (since the teacher is the authority on relevance).

By concentrating the limited teacher evaluations on the most promising documents (as predicted by the surrogate), this approach ensures that we find as many relevant documents as possible (high recall) while spending very few evaluations on irrelevant ones (maintaining precision). Importantly, because the teacher always evaluates documents with respect to the original query $Q$, it provides a stable reference point that prevents the system from drifting into evaluating documents that might only be relevant to a misconstrued reformulation. Any document that is irrelevant to $Q$ (even if it matched some reformulation) will receive a low score from the teacher, and this feedback will teach the surrogate to down-weight the responsible reformulation in future iterations.

\subsection{Online Reformulation Section}

Algorithm 1 implements the core online relevance estimation loop of \approach{}, which adaptively selects documents for expensive reranking under a strict budget. 
Starting from the original query $Q$, the algorithm first generates a set of reformulated queries $\mathcal{Q}$ and retrieves a candidate pool $\mathcal{C}$ by issuing each reformulation independently to a first-stage retriever and unioning the results with the initial retrieval $R_0$. 
Each document $d \in \mathcal{C}$ is represented by a feature vector $\vec{x}_d$ encoding its relevance signals with respect to the reformulations and the original query. A linear surrogate model with weights $\mathbf{w}_t$ estimates the utility of each document via $s(d;\mathbf{w}_t)=\mathbf{w}_t^\top\vec{x}_d$. At each iteration, the algorithm selects a small batch of documents with highest estimated utility, subject to the remaining reranking budget $c$, and queries a strong teacher reranker $\psi$ (MonoT5) to obtain relevance judgments anchored to the original query. These teacher scores are then used to update the surrogate weights by minimizing a squared prediction error, effectively performing online feature selection over reformulations. Scored documents are removed from the candidate pool and added to the result set, and the process repeats until the budget is exhausted. Through this iterative loop, \approach{} concentrates limited reranking effort on documents retrieved by the most effective reformulations, thereby increasing recall while actively suppressing query drift.

\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}

\begin{figure}[t]
\begin{algorithm}[H]
\caption{Online Relevance Estimation in \approach{}}
\begin{algorithmic}
\Require Original query $Q$, initial retrieved pool $R_0$, batch size $b$, reranking budget $c$, 
feature vector $\vec{x}_d$ for each document $d$
\Ensure Scored result set $R_1$

\State $R_1 \gets \emptyset$ \Comment{Documents scored by the teacher}

\State $\mathcal{Q} \gets \textsc{Reformulate}(Q)$
\Comment{Generate reformulated queries}

\ForAll{$Q_i \in \mathcal{Q}$}
    \State $D_i \gets \text{BM25}(Q_i)$
\EndFor

\State $\mathcal{C} \gets R_0 \cup \bigcup_{i} D_i$
\Comment{Candidate pool (documents as arms)}

\State Initialize $\mathbf{w}_1 \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$, $t \gets 1$
\Comment{Surrogate weights and iteration counter}

\Do
    \State \textbf{for all} $d \in \mathcal{C}$:
    \State \hspace{1em} $s(d;\mathbf{w}_t) \gets \mathbf{w}_t^\top \vec{x}_d$
    \Comment{Estimated utility}

    \State $B \gets$ top-$b$ documents from $\mathcal{C}$ by $s(d;\mathbf{w}_t)$
    \State $B \gets B$ truncated to respect remaining budget $c$
    
    \If{$|B| > 0$}
        \State \textbf{for all} $d \in B$:
        \State \hspace{1em} $y_d \gets \psi(Q,d)$
        \Comment{Teacher reranking (MonoT5)}

        \State Update $\mathbf{w}_{t+1}$ by minimizing
        \[
            \sum_{d \in B} \tfrac{1}{2}\big(\psi(Q,d) - \mathbf{w}^\top \vec{x}_d\big)^2
        \]
    \EndIf

    \State $R_1 \gets R_1 \cup \{(d,y_d): d \in B\}$
    \State $\mathcal{C} \gets \mathcal{C} \setminus B$
    \State $t \gets t+1$

\doWhile{$|R_1| < c$ and $\mathcal{C} \neq \emptyset$}

\end{algorithmic}
\label{algo:cerberus}
\end{algorithm}
\vspace{-0.6cm}
\end{figure}

During this process, reformulations that lead to many low-quality documents will be recognized and down-weighted early. For example, if $Q_j$ is a reformulation that retrieves mostly irrelevant documents, those documents (when eventually selected for teacher feedback) will receive low $y_d$ scores, and the weight $w_j$ corresponding to $Q_j$’s BM25 feature will decrease (because the surrogate will learn that a high BM25 score on $Q_j$ doesn’t correlate with true relevance). Conversely, a reformulation that consistently retrieves relevant documents will achieve high teacher scores for those documents, pushing its weight upward. This adaptive reweighting is done implicitly through the linear model’s updates.

\subsubsection{Efficiency considerations}
Another important aspect is efficiency: by focusing on top-scoring candidates first, we maximize the chance of finding relevant documents early. If the budget $c$ is much smaller than $|\mathcal{C}|$, the surrogate’s guidance ensures we pick the likely-best candidates rather than randomly sampling the pool. This makes the most of each precious call to the teacher.

\subsection{Why \approach{} Works?}

\paragraph{Recall without drift.} Using multiple reformulations dramatically improves recall by casting a wide net. \approach{} harnesses this strength but counteracts the typical precision drop by continually aligning the search with the original query’s intent. The teacher (anchored on $Q$) serves as a constant check on relevance, and the surrogate learns to emphasize reformulations that yield $Q$-relevant results. Thus, we retain high recall and maintain focus, avoiding drift into irrelevant regions of the collection.

\paragraph{Efficient, budget-aware learning.} Our method treats teacher evaluations as a limited resource and optimizes their use. Even a relatively small number of teacher-guided iterations are sufficient to significantly improve ranking quality: the surrogate model quickly learns from each batch of feedback and generalizes that knowledge to the remaining candidates. This budget-aware learning means we never waste the teacher’s effort on clearly irrelevant results for too long as they get pruned out as soon as their lack of relevance is observed.


% The relative gains from \approach{} are agnostic to how reformulations are generated. This is because we treat reformulations as features in an adaptive optimization framework. In other words, the method does not rely on any specific generation strategy and its gains come from managing drift.

\paragraph{Generator-agnostic design.}  In our experiments and results (Section~\ref{sec:experiments}), we  demonstrate that across different reformulation generators, \approach{} consistently improves performance. This suggests that the dominant failure mode in multi-query retrieval is not the lack of good reformulations (most methods can produce some useful variants), but rather the inability to control the low quality ones. Our approach addresses that dominant failure mode directly.

\paragraph{Interpretability and analysis.} An appealing byproduct of our feature-based approach is that the learned weight vector $\mathbf{w}$ provides insights into the retrieval process. We can inspect the weights after the retrieval is done to see which reformulations (or aspects of the query) were most valuable. For example, a high weight on a particular $Q_i$ might indicate that a certain rephrasing or subtopic was key to finding relevant documents. Similarly, a low or negative weight for a reformulation would indicate that it was not helpful (perhaps it introduced drift). This interpretability can aid in debugging query reformulation systems and in understanding the aspects of a query that were truly important for satisfying the information need.

==> plots/latency.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}
        \pgfplotsset{
            latency plot style/.style={
                ybar,
                width=0.7\columnwidth,
                height=5.0cm,
                bar width=7pt,
                symbolic x coords={50,100},
                xtick=data,
                enlarge x limits=0.25,
                ymajorgrids=true,
                grid style={dashed, gray!20},
                ylabel style={font=\small},
                xlabel style={font=\small},
                tick label style={font=\small},
                legend style={
                    font=\footnotesize,
                    at={(0.5,-0.35)},
                    anchor=north,
                    legend columns=3
                },
                cycle list={
                    {fill=orange!70, draw=black!80}, % RankLLaMA
                    {fill=gray!60,   draw=black!70}, % GEns + RRF
                    {fill=blue!60,   draw=black!80}  % GEns + Approach
                }
            }
        }

        \begin{axis}[
            latency plot style,
            ylabel={Mean latency per query (ms)},
            xlabel={Re-ranking budget ($c$)},
            title={\textbf{Re-ranking Latency vs Budget}}
        ]

            % RankLLaMA
            \addplot coordinates {
                (50,10863.2)
                (100,17562.6)
            };

            % GEns + RRF
            \addplot coordinates {
                (50,1406.14)
                (100,1757.67)
            };

            % GEns + Approach
            \addplot coordinates {
                (50,1679.8)
                (100,1939.89)
            };

            \legend{RankLLaMA, GEns+RRF, GEns+\approach{}}

        \end{axis}
    \end{tikzpicture}

    \caption{Mean re-ranking latency per query (ms) at different re-ranking budgets. GEns-based methods are an order of magnitude faster than RankLLaMA, with \approach{} incurring only marginal overhead over RRF.}
    \label{fig:latency_reranking}
\end{figure}


==> plots/latency_log_old.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}
        \pgfplotsset{
            latency plot style/.style={
                ybar,
                width=0.65\columnwidth,
                height=5.0cm,
                bar width=7pt,
                symbolic x coords={50,100},
                xtick=data,
                enlarge x limits=0.25,
                ymajorgrids=true,
                grid style={dashed, gray!20},
                ylabel style={font=\small},
                xlabel style={font=\small},
                tick label style={font=\small},
                legend style={
                    font=\footnotesize,
                    at={(0.5,-0.35)},
                    anchor=north,
                    legend columns=3
                },
                cycle list={
                    {fill=orange!70, draw=black!80}, % RankLLaMA
                    {fill=gray!60,   draw=black!70}, % $GEns$ + RRF
                    {fill=blue!60,   draw=black!80}  % $GEns$ + Approach
                }
            }
        }

        \begin{axis}[
            latency plot style,
            ymode=log,
            log basis y=10,
            ylabel={Mean latency per query (ms, log scale)},
            xlabel={Re-ranking budget ($c$)},
            title={\textbf{Re-ranking Latency vs Budget}},
            ymin=1e3, ymax=3e4,
            log ticks with fixed point
        ]

            % RankLLaMA
            \addplot+[
                error bars/.cd,
                y dir=both,
                y explicit
            ] coordinates {
                (50,10863.2)+- (0,0.56)
                (100,17562.6)+- (0,0.56)
            };

            % $GEns$ + RRF
            \addplot+[
                error bars/.cd,
                y dir=both,
                y explicit
            ] coordinates {
                (50,1406.14)+- (0,0.39)
                (100,1757.67)+- (0,0.56)
            };

            % $GEns$ + Approach
            \addplot+[
                error bars/.cd,
                y dir=both,
                y explicit
            ] coordinates {
                (50,1679.8)+- (0,0.56)
            (100,1939.89  ) +- (0,0.56)
            };

            \legend{RankLLaMA, $GEns$+RRF, $GEns$+\approach{}}

        \end{axis}
    \end{tikzpicture}

    \caption{Mean latency per query (log scale) at different re-ranking budgets. Std-dev is small, hence not visible. }
    \label{fig:latency_reranking}
\end{figure}


==> plots/varying_reform.tex <==
\tikzset{
    baseline style/.style={color=gray, mark=*, mark options={scale=0.5, solid}, line width=0.5pt},
    approach style/.style={color=blue, mark=*, mark options={scale=0.5, solid}, line width=0.5pt},
    ensemble style/.style={dashed, mark=square*, mark options={scale=0.5, solid}},
    error style/.style={color=red, mark=triangle*, mark options={scale=0.5, solid}, line width=0.5pt}
}

\begin{figure}[t]
    \centering
    % --- Merged Plot (A+C) ---
    \begin{subfigure}{0.49\columnwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                width = 1.15\linewidth,
                height = 1.0\linewidth,
                grid = major,
                grid style = {dashed, gray!20},
                xlabel = {\# of reformulations},
                ylabel = {Recall@100},
                title={\small{Varying \# of reformulations}},
                title style={yshift=-1.5ex},
                symbolic x coords={0,3,5,10,15,25,50},
                xtick={0,3,5,10,15,25,50},
                enlarge x limits=0.05,
                ymin=0.45, ymax=0.62,
                legend to name=sharedlegend,
                legend columns=2,
                legend style={font=\scriptsize, cells={anchor=west}, draw=none, column sep=0.5em}
            ]
                % Baseline
                \addplot [baseline style] table [x index=0, y index=3, col sep=comma] {fig/varying_n_vs_performance.txt};
                \addlegendentry{GenQR}

                % Ensemble Baseline
                \addplot [baseline style, ensemble style] table [x index=0, y index=3, col sep=comma] {fig/genqr_ensemble_varying_n.txt};
                \addlegendentry{$GEns$}
                
                % \addlegendimage{error style}
                % \addlegendentry{\approach{} (Error)}

                % Approach 1
                \addplot [approach style] table [x index=0, y index=4, col sep=comma] {fig/varying_n_vs_performance.txt};
                \addlegendentry{GenQR + \approach{}}

                % Approach Ensemble
                \addplot [approach style, ensemble style] table [x index=0, y index=4, col sep=comma] {fig/genqr_ensemble_varying_n.txt};
                \addlegendentry{$GEns$ + \approach{}}
            \end{axis}
        \end{tikzpicture}
        \caption{Recall Analysis}
    \end{subfigure}
    \hfill
    % --- Error Plot (B) ---
    \begin{subfigure}{0.49\columnwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                width = 1.15\linewidth,
                height = 1.0\linewidth,
                grid = major,
                grid style = {dashed, gray!20},
                xlabel = {\#batches scored by $\psi$},
                ylabel = {Error},
                title={\small{Estimation Error}},
                title style={yshift=-1.5ex},
                symbolic x coords={1,2,3,4,5,6,7},
                xtick={1,2,3,4,5,6,7},
                enlarge x limits=0.05,
                ylabel near ticks,
            ]
                \addplot [error style] table [x index=0, y index=4, col sep=comma] {fig/error_plot.txt};
            \end{axis}
        \end{tikzpicture}
        \caption{Estimation Error}
    \end{subfigure}

    \vspace{1em}
    \ref{sharedlegend} % Shared legend at bottom
    
    \caption{Performance scaling (left) and estimation error (right) on TREC DL19. Legend: Solid lines = Single GenQR, Dashed lines = Ensemble.}
\end{figure}

==> reformopt_algorithm.tex <==
\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%

\begin{figure}[t]
\begin{algorithm}[H]
\caption{Online Relevance Estimation } 
\begin{algorithmic}
\Require Query $q$, initial retrieved pool $R_0$, batch size $b$, budget $c$,  number of batches to score $m$, features vector $\vec{x}_d$ for document $d$
\Ensure Scored pool $R_1$
\State $R_1 \gets \emptyset$ \Comment{Scored results}
\State Reformulate original query -  $\mathcal{Q}
\gets Reformulate(Q)$

\State $D_i = BM25(Q_i) =  \{d_{i1}, d_{i2}, \ldots, d_{ik}\}$ $\forall Q_i \in \mathcal{Q}$
\State $\mathcal{D}_q \gets \bigcup_{i=1}^{m} D_i \cup R_0$ \Comment{candidate documents (Arms)}
%\State $S \gets \emptyset$ \Comment{top ranked documents}
\State $\Vec{w}_1 \leftarrow N(0,1)$ , $t \gets 1$ \Comment{Initialize weight vector and timestep}
% \State $B \gets$ \Call{Score}{top $b$ from $A$, subject to $c$} \Comment{Using monoT5}
% \State $R_1 \gets R_1 \cup B$ \Comment{Add batch to results}
% \State $A \gets A \setminus B$ \Comment{Discard the batch from Arms}
% \State\HiLi $\Call{SetAff}{.} \gets 0$ \Comment{Initialize expected affinity scores}
\Do
%and $X_i = [x_1...x_n]$, $\forall d \in A $
% \State $X \gets [\vec{x_1}...\vec{x_l}]$ where $l=|A|$ \& $\vec{x_i}$- feature vector for document $d$  \Comment{Construct feature matrix features for documents}
%\frac{1}{m}  \sum_{i=1}^n w_i  X_{i}]

  \State $\mathcal{D}_q \gets  \textsc{UtilEst}(\Vec{w}_t,\vec{x}_d) $  $\forall d \in \mathcal{D}_q$  \Comment{Assign estimated utility}
  \State $B \gets$ \Call{Select}{top $b$ from $\mathcal{D}_q$, subject to $c$} \Comment{using \textsc{UtilEst}}
 
  %\State $S \gets$ \Call{Select}{top $s$ from $R_1$} \Comment{Select top $s$ ranked docs}
 % \State $A \gets  \Call{EstRel}{q,d,S} \quad \forall d \in A$  \Comment{Assign estimated relevance scores}

  % \State $U \gets top_u(\textsc{D2DAff}(A))$
  % \State $C \gets top_c(\textsc{Q2DAff}(A))$ \Comment{Create shortlists of candidates}

% \State\HiLii $\Call{SetAff}{d} \gets \Call{SetAff}{d} + \Call{SetAff}{d,R_1}, \quad \forall d \in F$ \Comment{\small{Update Exp. Aff. Scores using (\ref{eq:eaffm})}}
% \normalsize
% \State $F \gets \Call{InterSetAff}{q, d,S} \quad \forall d \in F$ \Comment{Assign interpolated set affinity scores}


%\State $B \gets$ \Call{Select}{top-$b$ from \{$U \cup C$\}, subject to $c$} 
% \State $B_2 \gets$ \Call{Select}{top-$l_2$, $EstRel$ scores from $A$, ; $l_1+l_2=b$}
\If{$|R_1| < c$} 
    \State $B \gets$ \Call{Score}{$B$, subject to $c$} \Comment{ rank using $ \psi$  e.g., monoT5}
    \State $\vec{w}_{t+1} \gets \min_{\vec{w}} \mathcal{E}(\vec{w}_t,q,d, \vec{x}_d)$ $\forall d \in B$
% \Else 
% \State  $B \gets$ \Call{LookUp}{\textsc{EstRel} scores} $ \forall d \in B$
\EndIf

% %\State $B \gets B_1 \cup  B_2 $  
\State $R_1 \gets R_1 \cup B$ \Comment{Add batch to results}
\State $\mathcal{D}_q \gets \mathcal{D}_q\setminus B$ \Comment{Discard batch from Arms}
\State $t \gets t+1$


\doWhile{$|R_1| < c$}
%\State $R_1 \gets R_1 \cup \Call{Backfill}{R_0, R_1}$ \Comment{Backfill remaining items}
\end{algorithmic}
\label{algo:cerberus}
\end{algorithm} 
\vspace{-1cm}
\end{figure}

==> tables/bright.tex <==
\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rrrrrrr|rr|rrr|r}
\toprule
& \multicolumn{7}{c|}{StackExchange} & \multicolumn{2}{c|}{Coding} & \multicolumn{3}{c|}{Theorem-based} & \multirow{2}{*}{\centering Avg.}\\
\cmidrule(r){2-8} \cmidrule(r){9-10} \cmidrule(r){11-13}
& Bio. & Earth. & Econ. & Psy. & Rob. & Stack. & Sus. & Leet. & Pony & AoPS & TheoQ. & TheoT. \\
\midrule
BM25  & 0.172  &  & 0.140 & &  &  &  &  &  &  &  &  & \\
BM25>>RankGPT-4o &  &  &0.221  & &  &  &  &  &  &  &  &  & \\
\midrule
MonoT5-base & 0.127 &  &  & &  &  &  &  &  &  &  &  & \\
RankLLaMA-7B &  &  &  & &  &  &  &  &  &  &  &  & \\
RankLLaMA-13B  &  &  &  & &  &  &  &  &  &  &  &  & \\
 \rank-7B &  &  &  & &  &  &  &  &  &  &  &  & \\
\rank-14B &  &  &  & &  &  &  &  &  &  &  &  & \\
\rank-32B &  &  &  & &  &  &  &  &  &  &  &  & \\
\sgar  & 0.339 & --- &0.241  &--- & --- &---  &---  & --- &---  &---  & --- & --- &--- \\
\name~(Ours) & 0.372 & --- &  &--- & --- &---  &---  & --- &---  &---  & --- & --- &--- \\

\bottomrule
\end{tabular}
}
\caption{nDCG@10}
\label{tab:bright}
\end{table*}




\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|rrrrrrr|rr|rrr|r}
\toprule
& \multicolumn{7}{c|}{StackExchange} & \multicolumn{2}{c|}{Coding} & \multicolumn{3}{c|}{Theorem-based} & \multirow{2}{*}{\centering Avg.}\\
\cmidrule(r){2-8} \cmidrule(r){9-10} \cmidrule(r){11-13}
& Bio. & Earth. & Econ. & Psy. & Rob. & Stack. & Sus. & Leet. & Pony & AoPS & TheoQ. & TheoT. \\
\midrule
BM25  & 0.201 & --- &0.160  &--- & --- &---  &---  & --- &---  &---  & --- & --- &--- \\
BM25>>RankGPT-4o & --- & --- &0.234  &--- & --- &---  &---  & --- &---  &---  & --- & --- &--- \\
\midrule
MonoT5-base  & 0.160 & --- &---  &--- & --- &---  &---  & --- &---  &---  & --- & --- &--- \\
RankLLaMA-7B  & --- & --- &---  &--- & --- &---  &---  & --- &---  &---  & --- & --- &--- \\
RankLLaMA-13B   & --- & --- &---  &--- & --- &---  &---  & --- &---  &---  & --- & --- &--- \\
 \rank-7B  & --- & --- &---  &--- & --- &---  &---  & --- &---  &---  & --- & --- &--- \\
\rank-14B  & --- & --- &---  &--- & --- &---  &---  & --- &---  &---  & --- & --- &--- \\
\rank-32B  & --- & --- &---  &--- & --- &---  &---  & --- &---  &---  & --- & --- &--- \\
\sgar  & 0.387 & --- &0.247  &--- & --- &---  &---  & --- &---  &---  & --- & --- &--- \\
\name~(Ours) & 0.402 & --- &---  &--- & --- &---  &---  & --- &---  &---  & --- & --- &--- \\

\bottomrule
\end{tabular}
}
\caption{Recall@10}
\label{tab:bright_recall}
\end{table*}

==> tables/dl1920.tex <==
\begin{table*}
    \centering
    \caption{Effectiveness comparison of \approach{} across different query reformulation methods on TREC DL19 and DL20 test sets. Significant improvements using paired t-test, $p<0.05$, with Bonferroni correction, over respective baselines marked with corresponding letters. Note that subscript: (F) generally denotes significance of the reformulation approach augmented with \approach{} over the RRF variant. The best scores are highlighted in bold.}
    \vspace{-1em}
    {\small
     \setlength{\tabcolsep}{8.5pt}
    \begin{tabular}{llrrrrrr}
        \toprule
        \multicolumn{1}{l}{}&\multicolumn{1}{c}{}&\multicolumn{3}{c}{$c=50$}&\multicolumn{3}{c}{$c=100$} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}
Dataset&Pipeline  & nDCG@10 & nDCG@c & Recall@c & nDCG@10 & nDCG@c  & Recall@c \\
    \midrule
     & \bf\textsc{Exhaustive Retrieval} & \\
     %\cmidrule{2-11}
\multirow{19}{*}{\textbf{DL19}} \cellcolor{white} & MonoT5 & 0.672 & 0.625& 0.512  & 0.672 & 0.611  & 0.599  \\
\cmidrule{2-8} 
  & BM25>>MonoT5 [B] &0.681  & 0.541 &0.389 & 0.699 &0.563   &0.488  \\
& \idnt w/ RM3 &0.678  & 0.557 &0.405 & 0.686 &0.572 &0.507  \\ 
\cmidrule{2-8} 
 % \cellcolor{white} & BM25 >>RankLlama [RL] &0.693  & 0.545 &0.389 & 0.718 &0.568   &0.488 \\
%& \idnt w/ RM3 &0.684  & 0.559 &0.405 & 0.709 &0.580 &0.507  \\ 
   
%     &     CSQE &0.  & 0. &0. & 0. &0. &0. &0. &0. &0. \\

% \rowcolor{reformoptgray}     &      CSQE+ \approach{} &0.  & 0. &0. & 0.741 &0.666 &\textbf{0.618} &0. &0. &0. \\
&   \bf\textsc{Query reformulation} & \\
&     GenQR (G) &0.669  & 0.553 &0.401 & 0.694 &0.574 &0.510  \\
&     GenQR + RRF (F) &0.668  & 0.547 &0.394 & 0.689 &0.569 &0.505  \\
\rowcolor{reformoptgray}    
\cellcolor{white} & GenQR+ \approach{} &0.692  &${}^{G}_{BF}$ \bf  0.600 & ${}^{G}_{BF}$\textbf{0.453} & 0.720 &${}^{G}_{BF}$ 0.617 &${}^{G}_{BF}$ \textbf{0.561}  \\
\cmidrule{2-8}
&     $GEns$ &0.697  & 0.563 &0.423 & 0.724 &0.587 &0.537 \\
&     $GEns + RRF$ [F] &0.706  & 0.548 &0.421 & 0.723 &0.575 &0.525 \\    
\rowcolor{reformoptgray}      
\cellcolor{white} &  $GEns$ + \approach{} &0.714  & ${}^{GE}_{BF}$ 0.622 &${}^{GE}_{BF}$ \textbf{0.487} & 0.733 & ${}^{GE}_{BF}$ \bf 0.634 & ${}^{}_{BF}$\textbf{0.584} \\ 
\cmidrule{2-8}
 &     $GEnsPRF$ [R]  & 0.683  & 0.547 &0.412 & 0.715 &0.564 &0.508 \\ 
 \rowcolor{reformoptgray}      
\cellcolor{white} &  $GEnsPRF$ + \approach{} & \bf  0.684  & \bf ${}^{R}_{B}$  0.592 &\bf ${}^{R}_{B}$  0.454 &  0.723 & \bf ${}^{R}_{B}$ 0.626 & \bf ${}^{R}_{B}$ 0.575 \\ 
\cmidrule{2-8}     
&  QA-Expand &0.708  & 0.613 &0.468 & 0.739 &0.633 &0.575  \\
& QA-Expand + RRF &0.740  & 0.616 &0.464 & 0.758 &0.626 &0.582  \\   
\rowcolor{reformoptgray}      
\cellcolor{white} &  QA-Expand + \approach{} &${}^{Q}_{B}$ \bf 0.756  & ${}^{Q}_{BF}$ \bf 0.672 & ${}^{Q}_{BF}$\textbf{0.526} & 0.750 & ${}^{Q}_{BF}$ 0.668 & ${}^{Q}_{BF}$ \textbf{0.629}  \\ 
\cmidrule{2-8}
& Query2Doc (QD) &0.737  & 0.627 &0.502 & 0.747 &0.630 &0.605 \\
\rowcolor{reformoptgray}              
\cellcolor{white} &  Query2Doc + \approach{} &0.745  & \bf ${}^{QD}_{B}$0.671 & \bf 0.538 & 0.748 & ${}^{QD}_{B}$ \textbf{0.673} &\textbf{0.639}  \\
%    &     MuGI &0.  & 0. &0. & 0.769 &0.699 &0.663 &0. &0. &0. \\
% &      MuGI+ \approach{} &0.  & 0. &0. & 0. &0. &\textbf{0.} &0. &0. &0. \\
%      &      Lamer &0.  & 0. &0. & 0.756 &0.673 &{0.643} &0. &0. &0. \\
%           &      Lamer+ \approach{} &0.  & 0. &0. & 0. &0. &\textbf{0.} &0. &0. &0. \\
%  &   Intents + \approach{} &  & & & 0.710 & 0.609 & \textbf{0.553} \\
\hline
%\cmidrule{2-11}
 % \cellcolor{white} & BM25>>MonoT5 [B] &0.681  & 0.541 &0.389 & 0.699 &0.563   &0.488&0.719 &0.697 &0.755  \\
 %   & \idnt w/ RM3 &0.682  & 0.560 &0.409 & 0.686 &0.574 &0.507 &0.728 &0.717 &0.786 \\    
& \bf\textsc{Exhaustive Retrieval} & \\
\cellcolor{white} \multirow{18}{*}{\textbf{DL20}}  & MonoT5 &0.649  & 0.592 &0.576 & 0.649 &0.593 &0.670  \\        
\cmidrule{2-8} 
&   \bf\textsc{Query Reformulation} & \\
 \cellcolor{white} & BM25>>MonoT5 [B] &0.675  & 0.559 &0.478 & 0.684 &0.581   &0.584 \\
   & \idnt w/ RM3 &0.686  & 0.583 &0.510 & 0.698 &0.608 &0.629  \\ 
\cmidrule{2-8}
& GenQR (G) &0.684  & 0.583 &0.525 & 0.699 &0.610 &0.638  \\
& GenQR + RRF (GR) &0.687  & 0.582 &0.522 & 0.706 &0.617 &0.644 \\
\rowcolor{reformoptgray}     
\cellcolor{white} &   GenQR+ \approach{} &0.714  & ${}^{G}_{BF}$ 0.634 &${}^{G}_{BF}$ \textbf{0.594} & 0.718 &${}^{G}_{BF}$ 0.643 &${}^{G}_B$ \textbf{0.675}  \\
\cmidrule{2-8}
&     $GEns$ (GE) &0.684  & 0.586 &0.538 & 0.695 &0.611 &0.649\\
& $GenQR_{en}$ + RRF  &0.680  & 0.568 &0.519 & 0.698 &0.604 &0.645 \\

\rowcolor{reformoptgray}     
\cellcolor{white} &  $GEns$ + \approach{} &0.696  & ${}^{GE}$ \bf 0.627 &${}^{GE}$ \textbf{0.591} & 0.714 &${}^{GE}$ 0.641& \textbf{0.671} \\ 
\cmidrule{2-8}
&     $GEnsPRF$ [R] &0.667  & 0.569 &0.520 & 0.696 &0.601 &0.625 \\ 
&     $GEnsPRF$ + \approach{}  & \bf ${}^{R}_{B}$ 0.708  & \bf ${}^{R}_{B}$ 0.628 &\bf ${}^{R}_{B}$ 0.572 &  0.709 &${}^{R}_{B}$ \bf 0.637 & ${}^{R}_{B}$ \bf  0.671 \\ 
\cmidrule{2-8}
& QA-Expand (Q) &0.697  & 0.606 &0.576 & 0.707 &0.622 &0.669  \\
& QA-Expand + RRF &0.716  & 0.608 &0.558 & 0.721 &0.634 &0.689 \\       
\rowcolor{reformoptgray}
\cellcolor{white} & QA-Expand + \approach{} &0.723  & ${}^{Q}_{BF}$ \bf 0.651 & \textbf{0.615} & 0.726 &${}^{Q}_{BF}$ 0.661 & ${}^{Q}_{BF}$ \textbf{0.714} \\
\cmidrule{2-8}
& Query2Doc (QD) &0.718  & 0.632 &0.596 & 0.727 &0.649 &0.688 \\
\rowcolor{reformoptgray} 
\cellcolor{white} &  Query2Doc + \approach{} &\textbf{0.733}  & \bf 0.662 & \bf 0.616 & \textbf{0.729} & ${}^{QD}$ \textbf{0.680} &\textbf{0.730}  \\
\bottomrule     
\end{tabular}
}
    \vspace{-1.em}
    \label{tab:main}
\end{table*}

==> tables/latency_rankllama.tex <==

\begin{table*}

\caption{Mean re-ranking latency per query (in ms) at different re-ranking budgets using RankLLaMA (pointwise ranker) vs \approach{} with MonoT5.   }
\label{tab:latency-ranklamma}
\begin{tabular}{rrrclccclll}
\toprule
& \multicolumn{4}{c}{time (in ms)}& \multicolumn{4}{c}{nDCG@c (Recall@c)}  \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} 
c   & RankLlama &  & $GEns + RRF$  & $GEns$  & RankLlama & RankZephyr & $GEns + RRF$  & $GEns$ \\ 
  &  &  &   & + \approach{} &  &  &   & + \approach{}\\
\midrule
50   & 10863.2  &   &1406.14 &  1679.8  & 0.545 (0.389)   & 0.536 (0.389)  & 0.548(0.421)& \bf  0.622(0.487)  \\
\hline
\multirow{1}{*}{100}   & 17562.6 & & 1757.67     &  1939.89 & 0.568 (0.488)    &  0.565 (0.488)    & 0.575(0.525) &  \bf 0.634 (0.584)
 \\
%   & &  &  & (4)    &   &   &  \\
% \cmidrule{3-8}
% % 250   &  &  &  &  (3) & 0.684 &0.761  &0.667  \\
% 250   &  & 32312.97 & 30539.78 &  16092.16(8) & 0.684 &0.761  &  0.719\\
% % 500    &   &   &   &   &  &   &  \\
% % 750  &   &    &   &   &  &   &  \\
% \cmidrule{3-8}
% \multirow{3}{*}{1000}  &   & 127617.45  & 120885.39   & 16327.25(8) & 0.854 &0.881 & 0.829\\
%  &   &   &  & 31939.78(16)  &    &  & 0.839   \\
%  &   &   &  & 64390.74(32)  &    &  & 0.853   \\

\bottomrule
\end{tabular}
\end{table*}





==> tables/msmarco-v2.tex <==
\begin{table}[hbt!]
    \centering
    \caption{Effectiveness comparison* of \approach{} across reformulation approaches on TREC DL21 and DL22 test sets. The letter in subscript or superscript shows significant improvements (using paired t-test, $p<0.05$, with Bonferroni correction) over the corresponding baseline. Note that subscript: (F) generally denotes significance of the reformulation approach augmented with \approach{} over the RRF variant. }
{
    \small
     \setlength{\tabcolsep}{2pt}
    \begin{tabular}{lp{2.7cm}rrrr}
        \toprule
        \multicolumn{1}{l}{}&\multicolumn{1}{c}{}&\multicolumn{2}{c}{$c=50$}&\multicolumn{2}{c}{$c=100$} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
Dataset &Pipeline  &   nDCG@c & Recall@c &   nDCG@c  & Recall@c \\
    \midrule
  %  \multirow{14}{*}{\textbf{DL21}} &  \bf{PRF Baseline}  \\
  %   \cellcolor{white} \multirow{14}{*}{\textbf{DL21}}  & MonoT5 &   \\
\cellcolor{white} \multirow{20}{*}{\textbf{DL21}} & \\ 
 \cellcolor{white} & BM25>>MonoT5 [B] & 0.436 & 0.242 & 0.433 & 0.331 \\
   & \idnt w/ RM3 &0.455 & 0.274 & 0.457 & 0.375  \\ 
     \cmidrule{2-6}
 % \cellcolor{white} & RankLlama>>MonoT5 &   \\

  
 %  & \idnt w/ RM3 & 0. & 0. & & 0.  \\ 
   
%     &     CSQE &0.  & \\

% \rowcolor{reformoptgray}     &      CSQE+ \approach{} & \\
& \multicolumn{5}{l}{\bf\textsc{Query reformulation }} \\
\cmidrule{2-6}
 &     GenQR & 0.388  & 0.222  &0.398  & 0.317 \\
 &     GenQR + RRF & 0.390  & 0.226  &0.407  & 0.324 \\
\rowcolor{reformoptgray}    
\cellcolor{white} &      GenQR+ \approach{} & ${}^{G}_{BF}$ 0.484 & \bf ${}^{G}_{BF}$ 0.299  & \bf ${}^{G}_{BF}$ 0.488 & ${}^{G}_{BF}$ \bf 0.403 \\
 \cmidrule{2-6}

              % &     $GEns$ &0.  & 0. &0. & 0.726 &0.594 &0.539 &0. &0. &0. \\

&     $GEns$ [GE] & 0.421 & 0.266 & 0.432 & 0.370 \\
&     $GEns+RRF$ [F]  & 0.390 & 0.232 & 0.424 & 0.350 \\      
\rowcolor{reformoptgray}     
\cellcolor{white} &     $GEns$+\approach{} & ${}^{GE}_{BF}$ \textbf{0.480}  & ${}^{GE}_{BF}$ \textbf{0.308} & ${}^{GE}_{BF}$ \bf 0.484 & ${}^{GE}_{BF}$  \bf 0.402  \\ 
 \cmidrule{2-6}

& $GEns$ + PRF  [R]  & 0.408  & 0.251 & 0.410 & 0.332 \\  
\rowcolor{reformoptgray}     
\cellcolor{white} & \idnt  + \approach{}  & \bf ${}^{R}_{B}$ 0.491 & \bf  ${}^{R}_{B}$ 0.315 & \bf ${}^{R}_{B}$  0.485 & \bf ${}^{R}_{B}$ 0.409 \\
\cmidrule{2-6}
  &     QA-Expand (Q) & 0.483  &  0.329 & 0.482 & 0.437 \\
&     QA-Expand + RRF [F] & 0.498  &  0.328 & 0.493 & 0.441 \\       
  \rowcolor{reformoptgray}    
\cellcolor{white} &     QA-Expand & & & &  \\
  \rowcolor{reformoptgray} 
\cellcolor{white}   & + \approach{} & ${}^{Q}_{BF}$ \bf 0.538  &   \bf ${}^{}_{BF}$ 0.356  & \bf ${}^{Q}_{BF}$ 0.523 & \bf 0.463 \\ 
\cmidrule{2-6}
 &  Query2Doc [QD] & 0.456 & 0.316 & 0.466 & 0.420\\
  &  Query2Doc +\\ 
  \rowcolor{reformoptgray} 
\cellcolor{white}  & \approach{} & \bf  0.531 ${}^{QD}_{B}$ & \bf 0.354 & \bf  0.533${}^{QD}_{B}$ & \bf  0.481 ${}^{QD}_{B}$\\
     %    &     MuGI &0.  & 0. &0. & 0.769 &0.699 &0.663 &0. &0. &0. \\

     % &      MuGI+ \approach{} &0.  & 0. &0. & 0. &0. &\textbf{0.} &0. &0. &0. \\

     %      &      Lamer &0.  & 0. &0. & 0.756 &0.673 &{0.643} &0. &0. &0. \\

     %           &      Lamer+ \approach{} &0.  & 0. &0. & 0. &0. &\textbf{0.} &0. &0. &0. \\
          
  %  &   Intents + \approach{} &  & & & 0.710 & 0.609 & \textbf{0.553} \\
    \hline
\cellcolor{white} \multirow{18}{*}{\textbf{DL22}} & 
 BM25>>MonoT5 [B] & 0.290 & 0.115 & 0.275 & 0.164 \\
   & \idnt w/ RM3 &0. 287 & 0.115 & 0.275 & 0.161  \\   
  % & \idnt w/ RM3 &  & 0. & & 0.  \\ 
\cmidrule{2-6}
& \multicolumn{5}{l}{\bf\textsc{Query reformulation }} \\
\cmidrule{2-6}
&     GenQR (G) &0.292  & 0.136 & 0.288 & 0.193  \\
 &     GenQR + RRF &0.291  & 0.137 & 0.294 & 0.194  \\
\rowcolor{reformoptgray}     
\cellcolor{white} &      GenQR+\approach{} & \bf ${}^{G}_{BF}$ 0.352 & \bf  ${}^{G}_{BF}$ 0.170 & \bf ${}^{G}_{BF}$ 0.340 & \bf ${}^{G}_{BF}$ 0.236 \\
\cmidrule{2-6}
 % &     $GEns$ &0.  & 0. &0. & 0.726 &0.594 &0.539 &0. &0. &0. \\
&     $GEns$ (GE) &0.289 & 0.135 & 0.288 & 0.189 \\
&     $GEns + RRF$ (GE) &0.274 & 0.125 & 0.272 & 0.176 \\           
\rowcolor{reformoptgray}      
\cellcolor{white} &     $GEns$+\approach{} & \bf ${}^{GE}_{BF}$ 0.351 & \bf ${}^{GE}_{BF}$ 0.171 & \bf ${}^{GE}_{BF}$ 0.334 & \bf ${}^{GE}_{BF}$ 0.227  \\ 
\cmidrule{2-6}

& $GEns$ + PRF  [R]  & 0.251 & 0.100 & 0.248 & 0.145 \\  
\rowcolor{reformoptgray}     
\cellcolor{white} & \idnt  + \approach{}  & \bf 0.317 & \bf ${}^{R}_{B}$ 0.142 & \bf ${}^{R}_{B}$ 0.322  & \bf  ${}^{R}_{B}$ 0.213 \\
\cmidrule{2-6}

 &    QA-Expand &0.349  & 0.186 & 0.345 & 0.265\\
 &    QA-Expand + RRF [F] & 0.361  &  0.191 & 0.342 & 0.254 \\
\rowcolor{reformoptgray}     
\cellcolor{white} &     QA-Expand+\approach{} & \bf ${}^{Q}_{BF}$ 0.403 & \bf ${}^{Q}_{BF}$ 0.214  & \bf ${}^{}_{BF}$0.378 & \bf ${}^{}_{BF}$ 0.288\\
\cmidrule{2-6}
 &  Query2Doc  & 0.387 & 0.229 &0.366 & 0.306 \\
 \rowcolor{reformoptgray}      
\cellcolor{white} &  Query2Doc + & & & &\\
 \rowcolor{reformoptgray}      
\cellcolor{white} & \approach{} & \bf ${}^{QD}_{B}$ 0.425 & \bf  ${}^{}_{B}$ 0.240
  & \bf ${}^{QD}_{B}$ 0.410 & \bf ${}^{}_{B}$ 0.325 \\

\bottomrule
           
    \end{tabular}
    }
    \begin{minipage}{\columnwidth}
    \footnotesize{*We omit nDCG@10 our focus as prior works find that nDCG@10 value saturates quickly during re-ranking~\cite{plaid_repro}.}
\end{minipage}
    \label{tab:msmarcov2}
\end{table}


==> tables/small_llm_exp.tex <==
\begin{table}[hbt!]
    \centering
    \caption{Effectiveness comparison* of  \approach{} with different reformulator LLMs on TREC DL21 test set. The letter in subscript or superscript shows significant improvements (using paired t-test, $p<0.05$, with Bonferroni correction) over the corresponding baseline. Note re-ranker is MonoT5 unless otherwise explicitly specified }
{
    \small
     \setlength{\tabcolsep}{2pt}
    \begin{tabular}{lp{2.6cm}rrrr}
        \toprule
        \multicolumn{1}{l}{}&\multicolumn{1}{c}{}&\multicolumn{2}{c}{$c=50$}&\multicolumn{2}{c}{$c=100$} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
Dataset &Pipeline  &   nDCG@c & Recall@c &   nDCG@c  & Recall@c \\
    \midrule
  %  \multirow{14}{*}{\textbf{DL21}} &  \bf{PRF Baseline}  \\
     \cellcolor{white} \multirow{14}{*}{\textbf{DL21}}  & MonoT5 &   \\ 
     \cmidrule{2-6}
  %    &   \bf\textsc{Query reformulation } & \\
 \cellcolor{white} & BM25>>MonoT5 [B] & 0.436 & 0.242 & 0.433 & 0.331 \\
 
%   & \idnt w/ RM3 &0.455 & 0.274 & 0.457 & 0.375  \\ 

 \cellcolor{white} & BM25 >> RankLlama & 0.445 &0.242 & 0.438& 0.331   \\ 
 \cellcolor{white} & BM25 >> RankZephyr & 0.443 & 0.242 & 0.436 &0.331  \\
   
%     &     CSQE &0.  & \\

% \rowcolor{reformoptgray}     &      CSQE+ \approach{} & \\
      &   \bf\textsc{Llama 3.2:3b } & \\

         &     GenQR & 0.341  & 0.202  &0.368  & 0.301 \\
       &     GenQR + RRF & 0.351  & 0.202  &0.378  & 0.294 \\
\rowcolor{reformoptgray}     &      GenQR+ \approach{} & ${}^{G}_{BF}$ 0.471 & \bf ${}^{G}_{BF}$ 0.295  & \bf ${}^{G}_{BF}$ 0.466 & ${}^{G}_{BF}$ \bf 0.385 \\
              % &     $GEns$ &0.  & 0. &0. & 0.726 &0.594 &0.539 &0. &0. &0. \\

              &     $GEns$ [GE] & 0.405 & 0.154 & 0.283 & 0.223 \\
            &     $GEns+RRF$  & 0.257 & 0.141 & 0.309 & 0.222 \\       
\rowcolor{reformoptgray}      &     $GEns$+\approach{} & ${}^{GE}_{F}$ \textbf{0.449} & ${}^{GE}_{F}$ \textbf{0.276} & ${}^{GE}_{F}$ \bf 0.452 & ${}^{GE}_{F}$  \bf 0.372  \\ 

  %                   &     QA-Expand (Q) & 0.  &  0. & 0. & 0. \\
  %        &     QA-Expand + RRF & 0.  &  0. & 0. & 0. \\       
  % \rowcolor{reformoptgray}    &     QA-Expand + \approach{} & ${}^{Q}_{B}$ \bf 0. &   \bf  0. & \bf ${}^{Q}_{B}$ 0. & \bf 0. \\ 
     %    &     MuGI &0.  & 0. &0. & 0.769 &0.699 &0.663 &0. &0. &0. \\

     % &      MuGI+ \approach{} &0.  & 0. &0. & 0. &0. &\textbf{0.} &0. &0. &0. \\

     %      &      Lamer &0.  & 0. &0. & 0.756 &0.673 &{0.643} &0. &0. &0. \\

     %           &      Lamer+ \approach{} &0.  & 0. &0. & 0. &0. &\textbf{0.} &0. &0. &0. \\
          

  %  &   Intents + \approach{} &  & & & 0.710 & 0.609 & \textbf{0.553} \\

    %\hline
    % \cellcolor{white} \multirow{14}{*}{\textbf{DL22}}  & MonoT5 &   \\ 
     \cmidrule{2-6}
  %    &   \bf\textsc{Query reformulation } & \\
 % \cellcolor{white} & BM25>>MonoT5 [B] & 0.436 & 0.242 & 0.433 & 0.331 \\
 

 
 %  & \idnt w/ RM3 &0.455 & 0.274 & 0.457 & 0.375  \\ 

 % \cellcolor{white} & RankLlama>>MonoT5 &   \\

  
 %   & \idnt w/ RM3 & 0. & 0. & & 0.  \\ 
   
%     &     CSQE &0.  & \\

% \rowcolor{reformoptgray}     &      CSQE+ \approach{} & \\
      &   \bf\textsc{Qwen 2.5:3b } & \\

         &     GenQR & 0.353  & 0.214  &0.353  & 0.290 \\
       &     GenQR + RRF & 0.337 & 0.205 & 0.362 & 0.288\\
\rowcolor{reformoptgray}     &      GenQR+ \approach{} & ${}^{G}_{B}$ 0.457 & \bf ${}^{G}_{B}$ 0.282  & \bf ${}^{G}_{B}$ 0.458 & ${}^{G}_{B}$ \bf 0.371 \\
              % &     $GEns$ &0.  & 0. &0. & 0.726 &0.594 &0.539 &0. &0. &0. \\

              &     $GEns$ [GE] & 0.246 & 0.134 & 0.260 & 0.202 \\
            &     $GEns+RRF$  & 0.254 & 0.133 & 0.309 & 0.226 \\       
\rowcolor{reformoptgray}      &     $GEns$+\approach{} & ${}^{GE}_{B}$ \textbf{0.455} & ${}^{GE}_{B}$ \textbf{0.281} & ${}^{GE}_{B}$ \bf 0.448 & ${}^{GE}_{B}$  \bf 0.361  \\ 

\cline{2-6}

     &   \bf\textsc{Qwen 2.5:0.5b } & \\

         &     GenQR & 0.292  & 0.168  &0.319  & 0.248 \\
       &     GenQR + RRF & 0.357 & 0.201 & 0.371 & 0.288 \\
\rowcolor{reformoptgray}     &      GenQR+ \approach{} & ${}^{G}_{B}$ 0.467 & \bf ${}^{G}_{B}$ 0.289  & \bf ${}^{G}_{B}$ 0.445 & ${}^{G}_{B}$ \bf 0.366 \\
              % &     $GEns$ &0.  & 0. &0. & 0.726 &0.594 &0.539 &0. &0. &0. \\

              &     $GEns$ [GE] & 0.361 & 0.203 & 0.371 & 0.293 \\
            &     $GEns+RRF$  & 0.420 & 0.234     & 0.416 & 0.322 \\       
\rowcolor{reformoptgray}      &     $GEns$+\approach{} & ${}^{GE}_{B}$ \textbf{0.473} & ${}^{GE}_{B}$ \textbf{0.294} & ${}^{GE}_{B}$ \bf 0.449 & ${}^{GE}_{B}$  \bf 0.360  \\ 
\cline{2-6}

     &   \bf\textsc{Qwen 2.5:32b } & \\

         &     GenQR & 0.346  & 0.213  &0.353  & 0.289 \\
       &     GenQR + RRF & 0.330 & 0.209 & 0.359 & 0.301 \\
\rowcolor{reformoptgray}     &      GenQR+ \approach{} & ${}^{G}_{B}$ 0.489 & \bf ${}^{G}_{B}$ 0.313  & \bf ${}^{G}_{B}$ 0.488 & ${}^{G}_{B}$ \bf 0.413 \\
              % &     $GEns$ &0.  & 0. &0. & 0.726 &0.594 &0.539 &0. &0. &0. \\

 & $GEns$ [GE] & 0.375 & 0.240 & 0.379 & 0.317 \\
&  $GEns+RRF$  & 0.374 & 0.232     & 0.386 & 0.318     \\       
\rowcolor{reformoptgray}      &     $GEns$+\approach{} & ${}^{GE}_{B}$ \textbf{0.495} & ${}^{GE}_{B}$ \textbf{0.316} & ${}^{GE}_{B}$ \bf 0.487 & ${}^{GE}_{B}$  \bf 0.412  \\ 

\midrule
           
\end{tabular}
}
    \begin{minipage}{\columnwidth}
    \footnotesize{*We omit nDCG@10 our focus as prior works find that nDCG@10 value saturates quickly during re-ranking~\cite{plaid_repro}.}
\end{minipage}
    \label{tab:llm_exp}
\end{table}

